Edge-selective reconfiguration in polarized lattices with magnet-enabled bistability

The signature topological feature of Maxwell lattices is their polarization, which manifests as an unbalance in stiffness between opposite edges of a finite domain. The manifestation of this asymmetry is especially dramatic in the case of soft lattices undergoing large nonlinear deformation under concentrated loads, where the excess of softness at the soft edge can result in the activation of sharp indentations. This study explores how this mechanical dichotomy between edges can be tuned and possibly extremized by working with soft magneto-mechanical metamaterials. The magneto-mechanical coupling is obtained by endowing the lattice sites with permanent magnets, which activate a network of magnetic forces that can interact with (either augmenting or competing with) the elasticity of the material. Specifically, under sufficiently large deformation that macroscopically alters the equilibrium positions of the sites, the attractive forces between the magnets can trigger bistable reconfiguration mechanisms. The strength of such mechanisms depends on the landscapes of elastic reaction forces exhibited by the edges, which are different due to the polarization, and is therefore inherently edge-selective. We show that, on the soft edge, the addition of magnets simply enhances the softness of the edge. In contrast, on the stiff edge, the magnets activate snapping mechanisms that locally reconfigure the cells and produce a lattice response reminiscent of plasticity, characterized by residual deformation that persists upon unloading.

==> sections/Section02.tex <==
\section{Framework} \label{sec:develop}
Taking a step back and retracing the base topological theory that defines mathematically the rise of the stiff-soft edge dichotomy a revision of the underlying theory is needed.
The stiffness and consequential softness of a topologically polarized lattice can be assumed from the base cell that composes the finite system, it is in fact the truncated periodicity that gives rise to the topological localization and hence the different edge behaviours. 
Lattices that show topological polarization are described by means of a polarization vector ($R_{T}$) that is defined by the geometric (lattice vectors) and kinematic characteristics (compatibility matrix) of the lattice unit cell as reported in equations \ref{eq:top_1}, \ref{eq:top_2}. \textbf{need cit}

\begin{equation}
    R_{T} = \sum_{i} n_i \mathbf{a}_i
    \label{eq:top_1}
\end{equation}

\begin{equation}
    n_i = \frac{1}{2 \pi i } \oint_{C_i} d \mathbf{q} \cdot \nabla_q \text{ln}\left[\text{det}(C(\mathbf{q}))\right]
    \label{eq:top_2}
\end{equation}

Here $\mathbf{a}_i$ are the primitive lattice vectors and $n_i$ are the i winding numbers. C is the compatibility matrix of the unit cell parameterized to the wavevectors $\mathbf{q}$.
This calculation is not straight forward and it can become quite challenging in various instances. More importantly the result can be hard to predict and even harder to understand.
For this reason a tentative simplified equivalent theory for defining lattice polarization was proposed and reported here, so that an unambiguous soft-stiff edge polarization solution for these lattices can be defined a priori while also defining a loading indentation force direction that is compatible with the lattices in exam. The first component is important given the necessity of expanding the reasoning for stiffness induced polarization effects, especially when the present topological theory give an undetermined or hard grasp result. The second component is important in general for the study of topological effects, but most importantly here where bistability triggered effect are directional and trivial results can distort the final configuration that the structure can reach.
The main focus of the work was directed towards the detection of dichotomous behavior of the structural topological lattice when indented, both with and without embedded magnets in it. The presence of embedded magnets in an attractive configuration in the lattice was studied to see whether the bistable configuration of the cell could be triggered by ether one of the soft or stiff edges.
To study the effects of introducing reconfiguration driven by magnetic forces in polarized kagome lattices a conceptual problem had to be solved before starting the analyses: what kind of force directions are admissible for the indenter so that the result is a topologically driven response? 
To do so the following chapter will discuss a tentative simplified polarization theory devised to better describe and understand polarization by using a simplified approach.

\begin{figure*}[ht!]
\centering
\includegraphics[width = 0.9\textwidth]{sections/Figura_1.png}
\caption{(a) Rendering of a generic kagome structural lattice. On top the schematic representation of the same kagome cell but described by hinges and trusses.
(b) Reports the view from above of the same structure, highlighting the base cell vectors $b_1$ and $b_2$. (c) Reports the same lattice but highlighting the PT triangle and the center of mass. (d) Reports the kinematic representation of the cell when the PT triangle is loaded with a force that probes the topological properties of the cell. }
\label{fig:intro}
\end{figure*}

==> sections/Section_02.tex <==
\section{Framework} \label{sec:develop}
The main focus of the work is directed towards the detection of dichotomous behavior of the structural topological kagome lattice when indented, both with and without embedded magnets in it. The presence of embedded magnets in an attractive configuration in the lattice is studied to see whether the bistable configuration of the cell can be selectively triggered by ether one of the soft or stiff edges.
To study these effects a conceptual problem had to be solved before starting the analyses: what kind of force directions are admissible so that the result is a topologically driven response and not trivial behaviour.
To answer this, a deep study of the non linear kinematics of the lattice cell was conducted. These analyses also shed light into the overall kagome deformation and intrinsic directional stiffness. In light of these findings a new phenomenological polarization theory is devised and here presented, capable of bridging kinematics with statics. 

==> sections/section_top_theory.tex <==
\section{A simplified mechanistic perspective on polarization} \label{sec:top_teory}
%\subsection{Introduction} 

\begin{figure*}
\centering
\includegraphics[width = 1\textwidth]{sections/nuova_figura_1_FInale.png}
\caption{ (a,b,c) Macrocell of polarized kagome lattice encompassing six triangles and encapsulated hexagonal void. (a) Key geometric features and kinematic assumption on force direction required to filter out trivial responses. (b) Equivalent truss model of macrocell. (c) Deformed configuration of truss model highlighting activated degrees of freedom. (d,e,f) Workflow for the inference of stiff and soft edges induced by polarization. (d) Partition of the hexagonal void perimeter into six segments, each anchoring the center piece a three-rod truss, corresponding to six possible lattice edges (that can be realized, via bond severing, in the act of cutting a finite domain from an infinite lattice). (e) Diagram depicting the six possible trusses/edges, each with the appropriate load direction highlighted, and, at the center, the landscape of six reaction forces resulting from the analysis of the six edges. (f) The landscape of forces allows identifying and ranking the weakest egde(s), from which a ``stiffness direction" of the macrocell that correlates to the topological polarization vector can be inferred. (g) The analysis is compared against the family of kagome lattices studied in~\cite{rocklin2017transformable}, and repeated for different twist angles spanning the polarized and non-polarized regimes in polarization diagram; the reaction force landscapes predict directions of polarization consistent with topological theory in the polarized region of the diagram offer reliable, albeit heuristic criteria to determine the boundaries between polarized and non-polarized regimes.}
\label{fig:intro}
\end{figure*}

The main objective of this study is to document experimentally the onset of dichotomous behavior of a structural topological kagome lattice under sharp edge loads, with and without embedded magnets. Specifically, we intend to understand whether the embedding of magnets can selectively trigger bistable configurations at the edges and determine which edge (soft or stiff) is more amenable to this transition. One of the challenges arising in designing a framework to capture this behavior experimentally is determining how to load the edges in a way that truly elicits the topological character of the bulk instead of merely activating any trivial compliance of the edges. This issue, while fairly inconsequential for the small loads involved in linear elastic problems, becomes critical when dealing with large deformation of soft specimens \cite{widstrand2024robustness,pishvar2020soft,jolly2023soft}.
These considerations compel us to seek a deeper \textit{mechanistic} understanding of how the neighborhood of an edge cell subjected to loading deforms, and how this deformation penetrates in the bulk. Through this exercise, we
seek to build an intuitive framework to predict the polarization (or lack thereof) of a given kagome configuration only relying on geometric and kinematic considerations. 
While the proposed approach is deliberately pragmatic and does not claim to capture the topological attributes of a lattice, it does provide a simplified, yet reliable way to predict the availability of polarization. Therefore, 
it can provide a powerful complement to the formal theory of topological polarization, serving a practical purpose reminiscent of the model-free method to predict polarization recently put forward by Guzman et al.~\cite{hammer_Guzman}.


Let us consider a macrocell of kagome cells nearing an edge, consisting of one hexagonal void encapsulated by six triangles, as shown in Fig. \ref{fig:intro}(a). We will show that the lattice structural properties are effectively determined by the geometric features of the void. We make the assumption that the lattice can be described as a truss, i.e., a collection of rods linked by ideal hinges. A second important phenomenological assumption is that the load is applied as a force vector passing through the mid point of the interior side of the loaded triangle (along the perimeter of the void) and directed towards the centroid %center of mass% 
of the macrocell, % (see Fig. \ref{fig:intro}(a)). 
a choice of orientation that guarantees balance of angular momentum, avoiding %, while other load directions would result in 
rotations of the entire cell and/or the loaded triangle. 
This assumption is dictated by an explicit attempt to minimize possible activation of trivial edge effects, which typically involve isolated rotations of the edge triangles. %, thus filtering out the specific shape of the loaded triangle from the factors that significantly affect deformation.
We then proceed to select a loading triangle (labeled PT in Fig. \ref{fig:intro}(a)), which automatically selects the specific edge (among the many that can be realized by severing a finite domain from an infinite lattice) along which we intend the load to be applied. %model the application of loads. 

This treatment results in a simplified model of the macrocell under loading, shown in Fig. \ref{fig:intro}(b), that captures the salient cell kinematics. The two vertices bounding PT are modeled as internal hinges, while the next pair down is taken to behave as rollers constrained to slide along their connecting line. We neglect the bottom pair of hinges, since visual inspection of deformation fields from simulations and experiments on soft prototypes suggest that they generally do not move appreciably. This simplification is also inspired by a conceptual consideration regarding the purpose of our model: since we want to capture a surface mode that decays exponentially into the bulk, we can assume (with some reasonable approximation) that the degree of penetration of the deformation field into the bulk decays indeed within the first couple of cells. Two linear springs with constant $k$ model the lateral reaction forces exerted onto the macrocell by its neighbors. The outcome %of this modeling process 
is a 1-DOF system whose parameters are reported in Fig. \ref{fig:intro}(b): $L_1$ and $L_2$ are the lengths of the lateral rods, $\alpha$ and $\beta$ are the inclinations of the rods from the roller plane, and $\gamma$ is the angle between the roller plane and the PT rod $L_3$; $\Omega$ is the angle between the roller plane and the direction of loading; %applied displacement; 
$\Delta_1$ and $\Delta_2$ are the displacements of roller 1 and 2, respectively. A similar three-rod truss model with two hinges and two rollers can be constructed for any triangle around the void, thus modeling the kinematics of all possible edges that could exist at the boundary of a finite lattice.

It is now possible to evaluate the restoring force exhibited by each of the six possible edges under an imposed displacement $\delta$ applied to the PT, as shown in Fig. \ref{fig:intro}(c). The displacements of the rollers 
can be expressed as: 
\begin{equation}
\begin{aligned}
    \Delta_1 = L_1 [\cos(\alpha_f)-\cos(\alpha)]\\
    \Delta_2 = L_2 [\cos(\beta_f)-\cos(\beta)]
    \end{aligned}
\label{eq:00}
\end{equation}
where $\alpha_f$ and $\beta_f$ are the updated $\alpha$ and $\beta$ upon application of imposed displacement $\delta$. Note that the constraint on the loading direction ensures that $\gamma$ remains constant. Accordingly, Eq.~\ref{eq:00} is rewritten as: 
\begin{equation}
    \Delta_i = L_i \left \{ \cos \left[ \sin^{-1} \left( \sin( \chi_i)-\frac{\delta}{L_i} \cos(\Omega) \right) \right] -\cos(\chi_i) \right \}\\
\label{eq:044}
\end{equation}
where $\chi_i=\alpha , \beta$. Finally, from work balance considerations, the reaction force generated by the rollers is: 
\begin{equation}
    F = \frac{1}{\delta} \left( \frac{1}{2} k \Delta_1 ^ 2 + \frac{1}{2} k \Delta_2 ^ 2 \right) = \frac{k}{2 \delta}  \left( \Delta_1 ^ 2 + \Delta_2 ^ 2 \right)
\label{eq:03}
\end{equation}
According to Eq.~\ref{eq:03}, since $\Delta_1$ and $\Delta_2$ vary with the edge selection, each edge will respond with a different reaction force $F$ under the same imposed displacement $\delta$: the higher the reaction force, the stiffer the edge. This process is illustrated in Fig.\ref{fig:intro}(d,e,f), using the benchmark example of the kagome lattice discussed in~\cite{rocklin2017transformable}, for which the polarization vector direction is known. 
Moving along the macrocell void, we recognize the truss connections corresponding to the six possible edges (Fig.~\ref{fig:intro}(d)). For each, we resolve the kinematics shown in the six quadrants of Fig.~\ref{fig:intro}(e) and we compute the reaction forces, combining them in the macrocell force landscape plot in the central inset of Fig.~\ref{fig:intro}(e). %Cycling trough the six possible three-rod chains along the void contour, for each we evaluate the stiffness of the corresponding triangle, as indicated in  Fig.~\ref{fig:intro}(e). % Finally the polarization vector as pointing towards the weakest edge, but skewed towards the second weakest edge (Fig. \ref{fig:05}(f)).\\

\begin{figure*}[t]
\centering
\includegraphics[width = 1\textwidth]{sections/Figura_1_exp.png}
\caption{(a,b,c) Experimental setup for force-control experiments. (a) Schematic of setup, showing specimen laid flat in a plexiglass case and pulley system to apply compressive load via dead weight, using a loading tip with V-shaped notch to prevent trivial local rotations of the loaded edge triangle. (b) Dead weight apparatus %at the end of the pulley system
designed for incremental weight addition. (c) Detail of a cell of the silicone rubber prototype, highlighting finite thickness ligaments at the hinges and through holes (to be filled with plastic or magnetic fillers). (d) Experimental force-displacement curves for the lattice without magnets (purely mechanical response) under concentrated load, highlighting dichotomy between the soft and stiff edge. The markers correspond to snapshots in the (e-h) insets. (e,f) Snapshots of deformed states for load applied applied at the soft edge, in the linear and non-linear elastic regimes, respectively, revealing large localized deformation in the neighborhood of the tip that progressively increases with the load. (g,h) Snapshots for load applied applied at the stiff edge, showing stiffer response in the linear regime and sharp transition to %large 
localized deformation when local buckling mechanisms are triggered.}
\label{fig:ex:01}
\end{figure*}

With the ability to assign a stiffness value to each of the possible six edges, the next challenge is to generate a single descriptor of polarization with a significance akin to that of the \textit{polarization vector} in topological theory. Intuition suggests that the direction of such polarization vector should point towards the softest edge among the six. However, while intuitive, this general assignment rule is insufficient. Comparing its outcome against predictions from formal topological analysis for known polarized configurations, we are able to identify the missing rules that make the criterion general and robust. As shown in Fig.~\ref{fig:intro}(f) for our benchmark lattice, we can see that, when the softest edge is adjacent to the second softest, the correct polarization vector lies along an intermediate direction between the two, with the exact angle left indeterminate. %, as shown in Fig.~\ref{fig:intro}(f). 
%A reasonable hypothesis is that the angle is proportional to the ratio between the two reaction force vectors, with a
A special case arises %arising 
when the two softest edges are adjacent and equally soft, in which case the polarization vector is positioned precisely between them.
The robustness of the method is showcased in Fig.~\ref{fig:intro}(g) in which we sweep the configuration space of our selected kagome family by varying the twist angle, mimicking the sweep performed in~\cite{rocklin2017transformable} to construct the polarization phase diagram. We can see, that, for a wide range of twist angles, the computed force landscapes and the two-softest-edges criterion predict correctly the direction and the inclination of the polarization vector, including the transition from left-leaning to right-leaning occurring at the configuration featuring perfectly horizontal bonds (transition form green- to blue-shaded region in Fig.~\ref{fig:intro}(g), following the color coding in~\cite{rocklin2017transformable}).

While the edge stiffness ranking criterion provides a robust prediction of polarization direction for lattices that are polarized (the shaded region in Fig.~\ref{fig:intro}(g)), for non-polarized lattices, for which the formal polarization vector is zero, the criterion still yields a general rule, but its interpretation requires additional heuristic considerations. 
%While the method provides a robust prediction of polarization direction for lattices that are polarized (the shaded region), for non-polarized lattices, i.e., for which the formal polarization vector is zero, the interpretation of the outcome is less straightforward. Here, the edge stiffness ranking rule still yields a general criterion, but its interpretation requires additional heuristic considerations. 
Specifically, sweeping the twist angle %in the kagome class of Fig.~\ref{fig:intro} 
to extreme values %that eliminate polarization, 
we find that we exit the polarization regime when the stiffness of a \textit{single} edge of the macrocell vastly exceeds the others; in our example, this threshold is heuristically identified with the condition when the outlier stiffest edge experiences a reaction force exceeding $4.5$ times the mean value of all the reaction forces in the macrocell. These transitional configurations correspond to the lower and upper bounds of the shaded region Fig.~\ref{fig:intro}(g). Interestingly, a similar loss of polarization is not observed if we can identify at least two very stiff edges, regardless of the jump in stiffness between them and the others. 
Another class of non-polarized lattices is the family of twisted kagome lattices, in which the twisted triangles are equilateral. In this case, the method does capture the lack of polarization, which manifests as a landscape of triangles featuring exactly the same stiffness, which renders the assignment of any specific direction of maximum softness intrinsically ambiguous.
%\textcolor{red}{Still a complete and general rule for detecting the loss of polarization is undefined but the results obtained show interesting affinity with the polarization theory.}






